Geometric Separability using Orthogonal Objects

Given a bichromatic point set $P=\textbf{R} \cup \textbf{B}$ of red and blue points, a separator is an object of a certain type that separates $\textbf{R}$ and $\textbf{B}$. We study the geometric separability problem when the separator is a) rectangular annulus of fixed orientation b) rectangular annulus of arbitrary orientation c) square annulus of fixed orientation d) orthogonal convex polygon. In this paper, we give polynomial time algorithms to construct separators of each of the above type that also optimizes a given parameter.

==> Smax.tex <==

\begin{thm}
	\label{Smaxx}
	A separating concentric square annulus of maximum width can be constructed in $O(n \log^2 n)$ time.
\end{thm}
%\noindent\textbf{Proof of Theorem \ref{Smaxx}}
\begin{pf}
	Let $S_{max}$ be a separating concentric square annulus of maximum width. $S_{max}$ contains four input points on its boundary as specified in observation~\ref{sqr2}. 
	Let $S$ be a  separating concentric square annulus of maximum  possible width. Let $S_{out}$ and $S_{in}$ represent the outer and inner square of $S_{max}$ respectively.
	\\If there are more than two fixed points on the boundary of $S_{max}$ then we can find $S_{max}$ in $O(n \log n)$ time by correctly guessing the defining points in $O(n)$ time and checking the validity of each of these in $O(\log n)$ time. Therefore assume $S_{max}$ contains a fixed point each on two opposite sides. If not, there exist two adjacent sides that do not contain any fixed point. Then we can move these two sides outwards along the diagonal until $S_{out}$ touches a point in $\mathcal{B}_{out}$ or $S_{in}$ touches a point in $\mathcal{R}_{in}$. Without loss of generality assume that $p_{1}$ and $p_{2}$ lie respectively on the left and right sides of $S_{max}$. There should be at least one point from $\mathcal{R}_{in}$. Assume $p_1 \in R_{in}$. Now there are two cases based on the point $p_2$.
	\begin{enumerate}
		
		\item \textbf{The point $p_2$ is from $\mathcal{B}_{out}$ :}
		A third defining point $p_{3}$ is a red point in $S_{out}$. We can correctly guess this point in $O(n)$ time. There are two cases,
		
		\begin{enumerate}[a]
			\item $p_{3}$ lies on the left edge of $S_{out}$: Now we know two defining points $p_1$ and $p_3$ that lie on the same side of the annulus. This will give us the width of $S_{max}$ and thus we know the four vertical lines that contain the left and right edges of ${S}_{out}$ and $S_{in}$. For a correct guess of defining points $p_1$, $p_2$ and $p_3$, $\mathcal{R}_{in}$ lies between the slabs defined by these lines. By observation \ref{sqr2}, we know that the fourth defining point $p_4$ lies on the top or bottom side of $S_{max}$. 
			If this is a blue point, then it lies on $S_{in}$ and it is the nearest blue point vertically from $\mathcal{R}_{in}$. If this is a red point, then it lies on $S_{out}$ and it is the nearest red point vertically from $\mathcal{B}_{out}$. In both the cases $p_{4}$ can be found in $O(\log n)$ time. 
			
			
			\item $p_3$ lies on the top edge of ${S}_{out}$: Now by $p_2$ and $p_3$ we know the top right corner of $S_{out}$ and hence the line containing one diagonal of $S_{out}$. The point where this line intersects the vertical line containing $p_1$ is the bottom left corner of $S_{in}$ . By observation \ref{sqr2}, if $p_4$ is a red point 
			then it lies on the top side or right side of $S_{in}$ . 
%			In the former case,
%			it is the blue point with minimum y-coordinate in the region bounded by the lines $XY$ and $YW$.
%			%and in the latter case, it is the red point with minimum x-coordinate in the region bounded by the lines $YW$ and $YZ$.
%			If it is a red point in $S_{out}$, then it is the red point with the lowest y-coordinate in the region formed by diagonal line segment, $YZ$ and the vertical line contain $p_{2}$.   \\
%			
			
		\end{enumerate}
		
		
		
		The argument is symmetric if the third defining point that we guess lies on the bottom edge.
		
		\item \textbf{The point $p_{2}$ is from $\mathcal{R}_{in}$} : 
		
		The case where there are two red defining points on $S_{in}$ and one of them lies on the left or right edge is similar to 1(a). Otherwise, we construct the rest of the annulus using similar function in concentric square annulus with minimum width. 
		
		Instead of guessing a defining point
		we use a technique to find the center $c$ of $S_{max}$ and the defining point $p$ that lies on the top or bottom edge of $S_{in}$ .
		Let $r$ be the radius of $S_{out}$ which is given by half the difference of x-coordinates of the left and right edges of $S_{out}$. Let $l$ be the vertical line at distance $r$ from left and right edges of $S_{out}$. The center of the annulus, $c$, should lie on $l$ on a segment $L$ of length at most $2r$. \\
		We define a function $f_{p}(c)$ for all $p \in \textbf{ B}$, $c \in l$ as follows.
		
		\begin{equation}
		f_{p}(c)=
		\left\{  \begin{array}{cc}
		\infty & if \hspace{5pt}y(t(B_{out})) < y(p) <\\
		& y(b(B_{out})) \\
		\infty & if \hspace{5pt}y(p) > y(t(B_{out}))$ and $\\
		&y(c)> (y(p)+(y(b(B_{out}))))/2\\
		\infty & if \hspace{5pt} y(p) < y(b(B_{out}))$ and $\\
		& y(c) < (y(t(B_{out}))+y(p))/2  \\
		|y(p)-y(c)| &  \hspace{10pt}     otherwise
		\end{array}	
		\right.
		\end{equation}
		
		intuitively, $f_{p}(c)$ gives the radius of the square centered at $c$ and contains $p$ on the top or bottom edge and contains all red points in $\mathcal{R}_{in}$ inside it. For a fixed $c$, a square centered at $c$ that contains $\mathcal{R}_{in}$ inside and all the blue points outside has radius at most $\min_{p\in \textbf{B}} f_p(c)$. Moreover, a square $S_{in}$ that minimizes the width has radius $max_{c \in L}(\min_{p\in \textbf{B}} f_p(c))$.
		
		It is easy to see that, for a given $p$ the graph of $f_p(c)$ is a straight line segment $L_p$ of slope $+1$ or $-1$. Hence $max_{c \in L}(\min_{p\in \textbf{B}} f_p(c))$ is the maximum value of the lower envelope in the arrangement of $L_p$, for all $p \in \textbf{B}$. Computing the lower envelope of an arrangement of $n$ line segments can be done in $O(n \log n)$ time~\cite{square}. 
		
	\end{enumerate}
	
	Thus, $S$ should have the defining points in one of a constant number of configurations. In the configuration as in case(1) above, we can correctly guess the defining points in $O(n \log n)$ time and each guess can be validated in $O(\log n)$ time. Then the total running time for this case is $O(n \log^{2} n)$. All other cases can be solved in less time. Thus a separating square annulus of minimum width can be computed in $O(n \log^{2} n)$ time.
	
\end{pf}

